Accurate Computation of Quantum Excited States with Neural Networks

We present a variational Monte Carlo algorithm for estimating the lowest excited states of a quantum system which is a natural generalization of the estimation of ground states. The method has no free parameters and requires no explicit orthogonalization of the different states, instead transforming the problem of finding excited states of a given system into that of finding the ground state of an expanded system. Expected values of arbitrary observables can be calculated, including off-diagonal expectations between different states such as the transition dipole moment. Although the method is entirely general, it works particularly well in conjunction with recent work on using neural networks as variational Ans\"atze for many-electron systems, and we show that by combining this method with the FermiNet and Psiformer Ans\"atze we can accurately recover vertical excitation energies and oscillator strengths on a range of molecules. Our method is the first deep learning approach to achieve accurate vertical excitation energies, including challenging double excitations, on benzene-scale molecules. Beyond the chemistry examples here, we expect this technique will be of great interest for applications to atomic, nuclear and condensed matter physics.

==> preamble.tex <==
%LATEX PACKAGES GO HERE
\usepackage{amsmath}
%\usepackage{mathabx}
\usepackage{amsfonts}
\usepackage[utf8]{inputenc}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{graphicx}
\usepackage{float}
\usepackage{hhline}
\usepackage{booktabs}
\usepackage{etoolbox}
\usepackage{bbm}
\usepackage{cleveref}
\usepackage{tabularx}
\usepackage{url}
\usepackage{subcaption}
\restylefloat{table}


%tikz stuff
\usepackage{tikz}
\usetikzlibrary{shapes,arrows}

%******
%NAMING CONVENTIONS
%Where possible please find the section of this preamble where a variable fits.
%We are usually using camelCase naming of latex commands
%We are abbreviating words when the meaning is still obvious e.g params 
%Please try to avoid duplication.
%Please try to define commands in terms of other commands (within reason).
%Please define commands in the preamble rather than the main text.

%ABOVE ALL PLEASE USING COMMANDS INSTEAD OF RAW SYMBOLS
%THIS ENABLES US TO EASILY CHANGE AND ADAPT SYMBOLS


%******
%general defs
\newcommand{\params}{\theta}
\newcommand{\complexNumbers}{\mathbb{C}}
\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\functionComposition}{\circ}
\newcommand{\kronDelta}{\delta}
\newcommand{\indicatorFunction}{\mathbbm{1}}

%commments.
\newcommand{\commentOut}[1]{}
\newcommand{\comment}[1]{#1}
%\newcommand{\comment}[1]{}
\newcommand{\alexmatthews}[1]{\textcolor{cyan}{\comment{\emph{AM:} #1}}}
\newcommand{\davidpfau}[1]{\textcolor{blue}{\comment{\emph{DP:} #1}}}
\newcommand{\jamesspencer}[1]{\textcolor{green}{\comment{\emph{JS:} #1}}}
\newcommand{\matthewfoulkes}[1]{\textcolor{purple}{\comment{\emph{MF:} #1}}}
\newcommand{\jamesmartens}[1]{\textcolor{orange}{\comment{\emph{JM:} #1}}}
\newcommand{\resolved}[1]{}
%\newcommand{\alexmatthews}[1]{}
%\newcommand{\davidpfau}[1]{}
%\newcommand{\jamesspencer}[1]{}
%\newcommand{\matthewfoulkes}[1]{}


%******
%wavefunction defs.
\newcommand{\waveFunc}{\psi}
\newcommand{\waveFuncParams}{\psi_{\params}}

\newcommand{\spin}{\sigma}
\newcommand{\individualPosition}{\mathbf{r}}
\newcommand{\position}{\mathbf{\individualPosition}}
\newcommand{\overallPosition}{\mathbf{R}}
\newcommand{\overallPositionSpace}{\mathcal{R}}
\newcommand{\electronState}{x}
\newcommand{\electronStateSpace}{\mathbb{X}}
\newcommand{\overallState}{\mathbf{X}}
\newcommand{\overallStateSpace}{\mathcal{X}}

\newcommand{\electronIndex}{u}
\newcommand{\electronIndexB}{v}
\newcommand{\electronIndexC}{w}
\newcommand{\numElectrons}{N}
\newcommand{\spinUp}{\uparrow}
\newcommand{\spinDown}{\downarrow}
\newcommand{\particleExchange}{P}
\newcommand{\positionExchange}{\tilde{\particleExchange}}
\newcommand{\representationExchange}{\bar{\particleExchange}}
\newcommand{\arrayExchange}{\overline{\overline{\particleExchange}}}
\newcommand{\exchangedWaveFunc}{\waveFunc'}
\newcommand{\hfOrbital}{\phi}
\newcommand{\hfOrbitalIndex}{\mu}
\newcommand{\hfMatrix}{Q}
\newcommand{\hfWaveFunc}{\waveFunc_{\text{HF}}}
\newcommand{\hfPositionFunc}{\chi}
\newcommand{\genericSpin}{s}
\newcommand{\numSpinUp}{\numElectrons_{\spinUp}}
\newcommand{\numSpinDown}{\numElectrons_{\spinDown}}
\newcommand{\positionWaveFunc}{\Psi}

%Physical quantities
\renewcommand{\time}{t}
\newcommand{\mass}{m}
\newcommand{\energy}{E}
\newcommand{\localEnergy}{{E_L}}
\newcommand{\potentialEnergy}{V}

\newcommand{\energyRv}{L}
\newcommand{\scoreRv}{\vec{S}}

%Quantum mechanical operators
\newcommand{\qmOperator}[1]{\hat{#1}}
\newcommand{\hamiltonian}{\qmOperator{H}}
\newcommand{\exchangeOp}{\qmOperator{\particleExchange}}
\newcommand{\observable}{\qmOperator{\mathcal{O}}}
\newcommand{\kinetic}{\qmOperator{\mathcal{K}}}
\newcommand{\potential}{\qmOperator{\mathcal{V}}}

%Neural network definitions
\newcommand{\equivariantFunc}{f}
\newcommand{\equivariantDimension}{W}
\newcommand{\numDetsPerSpinChannel}{D}
\newcommand{\rawSplitTensor}{T}
\newcommand{\splitTensorUp}{\rawSplitTensor^{\spinUp}}
\newcommand{\splitTensorDown}{\rawSplitTensor^{\spinDown}}
\newcommand{\splitIndexA}{\mu}
\newcommand{\splitIndexB}{\nu}
\newcommand{\splitIndexC}{\gamma}
\newcommand{\splitIndexD}{\alpha}
\newcommand{\splitIndexE}{\beta}

\newcommand{\preReshapeTensor}{M}
\newcommand{\affineWeights}{w}
\newcommand{\affineBias}{b}
\newcommand{\reshapedTensor}{Q}
\newcommand{\outputDeterminant}{d}
\newcommand{\finalCoefficients}{\alpha}
\newcommand{\outputFunction}{g}

\newcommand{\nonlinearity}{\phi}
\newcommand{\equivariantScalarA}{\gamma}
\newcommand{\equivariantScalarB}{\nu}
\newcommand{\oneVector}{\mathbbm{1}}
\newcommand{\identityMatrix}{\mathbb{I}}
\newcommand{\const}{c}

%terms for describing full equivariant layer
\newcommand{\numFeatures}{K}

\newcommand{\featureIndex}{\gamma}
\newcommand{\featureIndexB}{\mu}

\newcommand{\rankOneFeaturesIn}{x}
\newcommand{\rankOneFeaturesOut}{c}
\newcommand{\rankTwoFeaturesIn}{y}
\newcommand{\rankTwoFeaturesOut}{d}

\newcommand{\rankTwoCoupling}{Q}
\newcommand{\rankTwoBias}{l}

\newcommand{\rankOneCouplingA}{A}
\newcommand{\rankOneCouplingB}{B}
\newcommand{\rankOneCouplingC}{C}
\newcommand{\rankOneCouplingD}{D}
\newcommand{\rankOneBias}{b}

%******
%densities and probability defs.

%random variables 
\newcommand{\rv}{y}
\newcommand{\rvB}{x}

\newcommand{\rawDensity}{p}
\newcommand{\density}{\rawDensity(\rv ; \params)}
\newcommand{\densityUnorm}{\tilde{\rawDensity}(\rv ; \params)}
\newcommand{\normalizer}{Z(\params)}

%Linear algebra stuff
\newcommand{\genericMatrix}{\mathbf{A}}
\newcommand{\CMat}{\mathbf{C}}
\newcommand{\genericScalar}{\alpha}
\newcommand{\adjugate}{\operatorname{Adj}}
\newcommand{\subMatrixSubtract}{\backslash}
\newcommand{\cofactor}{\operatorname{Cof}}
\newcommand{\transformedGenericMatrix}{\tilde{\genericMatrix}}
\newcommand{\matrixSize}{M}
\newcommand{\permutation}{\pi}
\newcommand{\symmetricGroup}{S}
\newcommand{\matrixIndex}{i}
\newcommand{\matrixIndexB}{j}
\newcommand{\sign}{\operatornname{Sign}}
\newcommand{\permSign}{\operatorname{Sgn}}
\newcommand{\precond}{\mathcal{M}}
\newcommand{\genericTarget}{L}

\newcommand{\identity}{\mathbf{I}}
\newcommand{\cofMat}{\mathbf{C}}
\newcommand{\svdLeft}{\mathbf{U}}
\newcommand{\svdMiddle}{\mathbf{\Sigma}}
\newcommand{\svdRight}{\mathbf{V}}
\newcommand{\diag}{\operatorname{diag}}

\newcommand{\expect}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\expectp}[1]{\expect{p(\overallState)}{#1}}
\newcommand{\rayleighQuotient}{R}
\newcommand{\covariance}{\operatorname{Cov}}

%Permutation equivariance stuff.
\newcommand{\permutationGroup}{S_{\numElectrons}}
\newcommand{\spinGroup}{T_{\numElectrons}}
\newcommand{\genericFunction}{f}
\newcommand{\genericFunctionB}{g}
\newcommand{\genericFunctionC}{h}
\newcommand{\transformedOverallPosition}{\overallPosition^{(\permutation)}}
\newcommand{\preNonLinear}{\mathbf{x}}
\newcommand{\postNonLinear}{\mathbf{y}}
\newcommand{\equivariantMatrix}{\mathbf{A}}
\newcommand{\equivariantBias}{\mathbf{b}}

\newtoggle{arxivversion} 
%\usepackage[
%backend=biber,
%style=alphabetic,
%sorting=ynt
%]{biblatex}
% 
%\addbibresource{bibliography.bib}

% Stuff specific to this paper, rather than imported from old papers
\newcommand{\op}{\hat{\mathcal{O}}}
\newcommand{\psit}{\psi^\star}
\newcommand{\Psit}{\Psi^\star}

\newcommand{\Na}{N_\alpha}
\newcommand{\Nb}{N_\beta}
\newcommand{\braket}[1]{\langle #1 \rangle}

\newcommand{\overlap}{\mathbf{S}}
\newcommand{\opoverlap}{\hat{\mathbf{O}}}
\newcommand{\hoverlap}{\hat{\mathbf{H}}}
\newcommand{\opoverlapopt}{\hat{\mathbf{O}}^*}
\newcommand{\hoverlapopt}{\hat{\mathbf{H}}^*}

\newcommand{\psimat}{\mathbf{\Psi}}
\newcommand{\psimatopt}{\mathbf{\Psi}^{*}}

\newcommand{\oppsimat}{\hat{\mathcal{O}}\psimat}
\newcommand{\hpsimat}{\hat{H}\psimat}
\newcommand{\hpsimatopt}{\hat{H}\psimatopt}
